FrugalNeRF: Fast Convergence for Extreme Few-shot Novel View Synthesis without Learned Priors

Neural Radiance Fields (NeRF) face significant challenges in extreme few-shot scenarios, primarily due to overfitting and long training times. Existing methods, such as FreeNeRF and SparseNeRF, use frequency regularization or pre-trained priors but struggle with complex scheduling and bias. We introduce FrugalNeRF, a novel few-shot NeRF framework that leverages weight-sharing voxels across multiple scales to efficiently represent scene details. Our key contribution is a cross-scale geometric adaptation scheme that selects pseudo ground truth depth based on reprojection errors across scales. This guides training without relying on externally learned priors, enabling full utilization of the training data. It can also integrate pre-trained priors, enhancing quality without slowing convergence. Experiments on LLFF, DTU, and RealEstate-10K show that FrugalNeRF outperforms other few-shot NeRF methods while significantly reducing training time, making it a practical solution for efficient and accurate 3D scene reconstruction.

==> figs/dtu_depth.tex <==
\begin{figure}[h]
\vspace{-4mm}
\centering
\resizebox{0.95\columnwidth}{!} 
{
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=\textwidth]{figure_partition/teaser/pdf/CEVR.pdf}
% \includegraphics[width=\textwidth]{figures/Ablation_high_low_curve.png}
\includegraphics[width=\textwidth]{figures/DTU_depth.pdf}}
\label{fig:dtu_depth}
\vspace{-5mm}
\end{figure}

==> figs/mse_curves.tex <==
\begin{figure}[h]
\vspace{-4mm}
\centering
\resizebox{1.0\columnwidth}{!} 
{
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=\textwidth]{figure_partition/teaser/pdf/CEVR.pdf}
% \includegraphics[width=\textwidth]{figures/Ablation_high_low_curve.png}
\includegraphics[width=\textwidth]{figures/mse_diff.pdf}
}
%green curve is high res-voxel, pink one is low-res voxel 
%orange curve is mid res-voxel
\label{fig:mse_curves}
\vspace{-8mm}
\end{figure}

==> figs/psnr_curves.tex <==
% \begin{figure}[h]
% \vspace{-7mm}
% \centering
% \resizebox{1.0\columnwidth}{!} 
% {
% %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% % \includegraphics[width=\textwidth]{figure_partition/teaser/pdf/CEVR.pdf}
% % \includegraphics[width=\textwidth]{figures/Ablation_high_low_curve.png}
% \includegraphics[width=\textwidth]{figures/psnr_iter.pdf}
% }
% %green curve is high res-voxel, pink one is low-res voxel 
% %orange curve is mid res-voxel
% \label{fig:psnr_curves}
% \vspace{-11mm}
% \end{figure}
\hspace{-5mm}
\begin{minipage}{.57\linewidth}
\vspace{2mm}
\includegraphics[width=1.\linewidth]{figures/psnr_iter.pdf}
\end{minipage}
\resizebox{0.40\linewidth}{!}{%
\begin{tabular}{l|ccc}
\toprule
 & \multicolumn{3}{c}{2-view} \\
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
FreeNeRF [\textcolor{cvprblue}{76}] & \cellcolor{yellow!25}13.09 & \cellcolor{orange!25}0.55 & \cellcolor{orange!25}0.42\\
ViP-NeRF [\textcolor{cvprblue}{58}] & 12.23 & \cellcolor{yellow!25}0.51 & \cellcolor{yellow!25}0.46 \\
SimpleNeRF [\textcolor{cvprblue}{59}] & 7.60 & 0.28 & 0.74 \\
VGOS [\textcolor{cvprblue}{61}] & 7.92 & 0.26 & 0.74 \\ 
SparseNeRF [\textcolor{cvprblue}{67}] & \cellcolor{red!25}13.53 & \cellcolor{orange!25}0.55 & \cellcolor{orange!25}0.42 \\
Ours & \cellcolor{orange!25}13.32 & \cellcolor{red!25}0.58 & \cellcolor{red!25}0.40 \\
 \bottomrule
\end{tabular}%
}
% \vspace{-1mm}

==> figs/rebuttal_real_visual.tex <==
\begin{figure}[h!]
\centering
\vspace{-4mm}
\resizebox{1.0\columnwidth}{!} 
{
\includegraphics[width=\textwidth]{figures/rebuttal_real_visual.pdf}
}
% }
\vspace{-11mm}
\label{fig:rebuttal_real_vis}
\end{figure}

==> figs/scene_analysis.tex <==
\begin{figure}[h]
\vspace{-4mm}
\centering
\resizebox{1.0\columnwidth}{!} 
{
\includegraphics[width=\textwidth]{figures/scene__analysis.pdf}
}
\label{fig:scene__analysis}
\vspace{-8mm}
\end{figure}

==> figs/viewpoint_curves.tex <==
\begin{figure}[h]
\vspace{-4mm}
\centering
\resizebox{1.0\columnwidth}{!} 
{
\includegraphics[width=\textwidth]{figures/view_point.pdf}
}
\label{fig:viewpoint_curves}
\vspace{-9mm}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/abalation_with_mono_depth.tex <==
% % \begin{table*}[t]
% % \centering
% % \caption{\textbf{Comparisons on Adding a Pretrained Monocular Depth Prior.}}
% % \vspace{-2mm}
% % \label{tab:abalation_with_mono_depth}
% % \resizebox{\textwidth}{!}{%
% % \begin{tabular}{l|ccc|ccc|ccc}
% % \toprule
% %  & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c}{4-view} \\
% % Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$\\
% % \midrule 
% % SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 & 19.52 & 0.59 & 0.37 & 20.89 & 0.65 & 0.34 \\
% % FrugalNeRF & 18.07 & 0.54 & \bf{0.35} & 19.40 & 0.60 & 0.31 & 20.95 & 0.65 & 0.28 \\
% % FrugalNeRF w/ mono. depth & \bf{18.10} & \bf{0.55} & \bf{0.35} & 19.40 & 0.60 & 0.31 & 20.95 & 0.65 & 0.28 \\
% %  \bottomrule
% % \end{tabular}%
% % }
% % \end{table*}

% \begin{table*}[t]
% \centering
% \caption{\textbf{Comparisons on adding a pre-trained monocular depth prior.}}
% \vspace{-2mm}
% \label{tab:abalation_with_mono_depth}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccc}
% \toprule
%  % & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c}{4-view} \\
% Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS \\
% \midrule 
% SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 \\
% FrugalNeRF & 18.07 & 0.54 & \bf{0.35} \\
% FrugalNeRF w/ mono. depth & \bf{18.10} & \bf{0.55} & \bf{0.35}\\
%  \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{figure}[t]
% \centering
% \resizebox{1.0\columnwidth}{!} 
% {
% % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=\textwidth]{figures/mono_depth_viz.pdf}
% }
% \compress
% \compress
% \caption{\textbf{Visual comparisons on adding a pre-trained monocular depth prior.} 
% }
% \label{fig:mono_vis}
% \compress
% \end{figure}

% % Combining two tables
% \begin{table}[t]
%     \centering\small
%     \begin{minipage}[t!]{0.36\textwidth}
%         \centering
%         \small
%         \caption{\textbf{Comparisons on adding a pre-trained monocular depth prior.}}
%         \compress
%         \label{tab:abalation_with_mono_depth}
%         \resizebox{1.0\textwidth}{!}{%
%         \begin{tabular}{l|ccc}
%         \toprule
%          % & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c}{4-view} \\
%         Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS \\
%         \midrule 
%         SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 \\
%         FrugalNeRF & 18.07 & 0.54 & \bf{0.35} \\
%         FrugalNeRF w/ mono. depth & \bf{18.10} & \bf{0.55} & \bf{0.35}\\
%          \bottomrule
%         \end{tabular}%
%         }
%     \end{minipage}
%     \hskip1em
%     \begin{minipage}[t!]{0.60\textwidth}
%         % \centering
%         \resizebox{1.0\columnwidth}{!} 
%         {
%         % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%         \includegraphics[width=\textwidth]{figures/mono_depth_viz.pdf}
%         }
%         \compress
%         \compress
%         \caption{\textbf{Visual comparisons on adding a pre-trained monocular depth prior.} 
%         }
%         \label{fig:mono_vis}
%         \compress
%     \end{minipage}
% \compress
% \end{table}

\begin{table}[t]
\centering
\centering
\caption{\textbf{Comparisons on adding a pre-trained monocular depth prior.}}
\label{tab:abalation_with_mono_depth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule 
SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 \\
FrugalNeRF & 18.07 & 0.54 & \textbf{0.35} \\
FrugalNeRF w/ mono. depth & \textbf{18.10} & \textbf{0.55} & \textbf{0.35}\\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{figure}[t]
\centering
% \resizebox{1.0\columnwidth}{!}{%
\includegraphics[width=\columnwidth]{figures/mono_depth_viz.pdf}
% }
\caption{\textbf{Visual comparisons on adding a pre-trained monocular depth prior.}}
\label{fig:mono_vis}
\end{figure}


% \begin{table*}[t]
% \centering
% \begin{minipage}{0.48\textwidth}
% \centering
% \captionof{table}{Comparisons on adding a pre-trained monocular depth prior.}
% \label{tab:abalation_with_mono_depth}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccc}
% \toprule
% Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
% \midrule 
% SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 \\
% FrugalNeRF & 18.07 & 0.54 & \textbf{0.35} \\
% FrugalNeRF w/ mono. depth & \textbf{18.10} & \textbf{0.55} & \textbf{0.35}\\
% \bottomrule
% \end{tabular}%
% }
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \resizebox{1.0\textwidth}{!}{%
% \includegraphics[width=\textwidth]{figures/mono_depth_viz.pdf}
% }
% \captionof{figure}{Visual comparisons on adding a pre-trained monocular depth prior.}
% \label{fig:mono_vis}
% \end{minipage}
% \end{table*}



==> tables/ablation_shared_voxels.tex <==
% \begin{table}[t]
% \centering
% \small
% \caption{\textbf{Effect of voxels weight-sharing.}}
% % \caption{\textbf{Effect of voxels weight sharing on the \emph{scan21} scene in the DTU~\cite{jensen2014large} dataset with two input views.}}
% \vspace{-1mm}
% \label{tab:ablation_shared_voxels}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccccc}
% \toprule
%                    &PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Model size $\downarrow$ \\
% \midrule
% w/o           &   16.20   &   0.83  &  0.17    & 70.81 MB \\
% w/                  &   \bf{17.50}   &  \bf{0.85}  &  \bf{0.14} &  \bf{66.24 MB}  \\
% \bottomrule
% \end{tabular}%
% % }
% \end{table}
% \vspace{-2mm}

% % w/o 20.14 0.89 0.12
% % w/ 20.26 0.89 0.12
% % w/o           &   12.70   &   0.57  &  0.41    & 70.81 MB \\
% % w/                  &   \bf{13.32}   &  \bf{0.58}  &  \bf{0.40} &  \bf{66.24 MB}  \\


==> tables/quantitative_dtu_unmask.tex <==
% \begin{table}[h]
% \vspace{-6mm}
% \centering
% % \caption{\textbf{Quantitative results on the DTU~\cite{jensen2014large} dataset.} FurgalNeRF synthesizes better images than most of the other baselines under extreme few-shot settings but with shorter training time and does not rely on any externally learned priors.}
% \label{tab:quantitative_dtu}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
%  & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c}{4-view} \\
% Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
% \midrule
% FreeNeRF [\textcolor{cvprblue}{76}] & \cellcolor{yellow!25}13.09 & \cellcolor{orange!25}0.55 & \cellcolor{orange!25}0.42 & \cellcolor{red!25}15.70 & \cellcolor{red!25}0.66 & \cellcolor{red!25}0.31 & \cellcolor{red!25}18.64 & \cellcolor{red!25}0.74 & \cellcolor{red!25}0.25  \\
% ViP-NeRF [\textcolor{cvprblue}{58}] & 12.23 & \cellcolor{yellow!25}0.51 & \cellcolor{yellow!25}0.46 & 12.86 & 0.54 & 0.45 & 14.5 & 0.58 & 0.39 \\
% SimpleNeRF [\textcolor{cvprblue}{59}] & 7.60 & 0.28 & 0.74 & 8.30 & 0.30 & 0.71 & 10.16 & 0.37 & 0.62 \\
% VGOS [\textcolor{cvprblue}{61}] & 7.92 & 0.26 & 0.74 & 8.01 & 0.27 & 0.75 & 8.54 & 0.30 & 0.76\\ 
% SparseNeRF [\textcolor{cvprblue}{67}] & \cellcolor{red!25}13.53 & \cellcolor{orange!25}0.55 & \cellcolor{orange!25}0.42 & \cellcolor{orange!25}14.81 & \cellcolor{orange!25}0.64 & \cellcolor{orange!25}0.33 & \cellcolor{orange!25}16.39 & \cellcolor{orange!25}0.71 & \cellcolor{orange!25}0.28 \\
% Ours & \cellcolor{orange!25}13.32 & \cellcolor{red!25}0.58 & \cellcolor{red!25}0.40 & \cellcolor{yellow!25}14.76 & \cellcolor{yellow!25}0.60 & \cellcolor{yellow!25}0.38 & \cellcolor{yellow!25}16.28 & \cellcolor{yellow!25}0.69 & \cellcolor{yellow!25}0.32 \\
%  \bottomrule
% \end{tabular}%
% }
% \vspace{-4mm}
% \end{table}

\begin{table}[h]
\vspace{-3mm}
\centering
% \caption{\textbf{Quantitative results on the DTU~\cite{jensen2014large} dataset.} FurgalNeRF synthesizes better images than most of the other baselines under extreme few-shot settings but with shorter training time and does not rely on any externally learned priors.}
\label{tab:quantitative_dtu}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c}{4-view} \\
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
FreeNeRF [\textcolor{cvprblue}{76}] & 13.09 & 0.55 & 0.42 & 15.70 & 0.66 & 0.31 & 18.64 & 0.74 & 0.25  \\
ViP-NeRF [\textcolor{cvprblue}{58}] & 12.23 & 0.51 & 0.46 & 12.86 & 0.54 & 0.45 & 14.5 & 0.58 & 0.39 \\
SimpleNeRF [\textcolor{cvprblue}{59}] & 7.60 & 0.28 & 0.74 & 8.30 & 0.30 & 0.71 & 10.16 & 0.37 & 0.62 \\
VGOS [\textcolor{cvprblue}{61}] & 7.92 & 0.26 & 0.74 & 8.01 & 0.27 & 0.75 & 8.54 & 0.30 & 0.76\\ 
SparseNeRF [\textcolor{cvprblue}{67}] & 13.53 & 0.55 & 0.42 & 14.81 & 0.64 & 0.33 & 16.39 & 0.71 & 0.28 \\
Ours & 13.32 & 0.58 & 0.40 & 14.76 & 0.60 & 0.38 & 16.28 & 0.69 & 0.32 \\
 \bottomrule
\end{tabular}%
}
\vspace{-4mm}
\end{table}

==> tables/rebuttal_Real_2v.tex <==
\begin{table}[h!]
\centering
% \vspace{-3mm}
\small
\label{tab:real_rebuttal}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|c}
\toprule
 % & \multicolumn{3}{c|}{2-view} & Training \\
Method (RealEstate-10K) & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Training time $\downarrow$\\
\midrule
ViP-NeR [{\color{eccvblue}67}] & 29.55 & \cellcolor{orange!25}0.87 & 0.09 & 13.5 hrs\\
SimpleNeRF [{\color{eccvblue}66}] & \cellcolor{red!25}30.30 & \cellcolor{red!25}0.88 & \cellcolor{red!25}0.07 & 9.5 hrs\\
FrugalNeRF (Ours) (3 scales) & 28.90 & \cellcolor{orange!25}0.87 & \cellcolor{orange!25}0.08 & \cellcolor{red!25}8 mins\\
FrugalNeRF (Ours) (4 scales) & \cellcolor{orange!25}30.01 & \cellcolor{red!25}0.88 & \cellcolor{orange!25}0.08 & \cellcolor{orange!25}15 mins\\
 \bottomrule
\end{tabular}%
}
\end{table}


==> tables/rebuttal_monodepth.tex <==
% \begin{table}[h]
% \centering
% \begin{minipage}{0.48\textwidth}
% \centering
% \label{tab:abalation_with_mono_depth}
% \vspace{-2mm}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccc}
% \toprule
% Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
% \midrule 
% SparseNeRF~\cite{wang2023sparsenerf} &  18.02 & 0.52 & 0.45 \\
% FrugalNeRF & 18.07 & 0.54 & \textbf{0.35} \\
% FrugalNeRF w/ mono. depth & \textbf{18.10} & \textbf{0.55} & \textbf{0.35}\\
% \bottomrule
% \end{tabular}%
% }
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \resizebox{1.0\textwidth}{!}{%
% \includegraphics[width=\textwidth]{figures/mono_depth_viz.pdf}
% }
% \captionof{figure}{Visual comparisons on adding a pre-trained monocular depth prior.}
% \label{fig:mono_vis}
% \end{minipage}
% \end{table}


\begin{table}[h]
\centering
\vspace{-3mm}
\label{tab:real_rebuttal}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|c}
\toprule
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Training time $\downarrow$\\
\midrule
SparseNeRF [{\color{eccvblue}75}] &  18.02 & 0.52 & 0.45 & 1 hr\\
FrugalNeRF (Ours) & 18.07 & 0.54 & \textbf{0.35} & 10 mins\\
FrugalNeRF (Ours) w/ mono. depth & \textbf{18.10} & \textbf{0.55} & \textbf{0.35} & 11 mins\\
 \bottomrule
\end{tabular}%
}
\vspace{-3mm}
\end{table}
